Autonomous Extracting a Hierarchical Structure of Tasks in Reinforcement Learning and Multi-task Reinforcement Learning

Reinforcement learning (RL), while often powerful, can suffer from slow learning speeds, particularly in high dimensional spaces. The autonomous decomposition of tasks and use of hierarchical methods hold the potential to significantly speed up learning in such domains. This paper proposes a novel practical method that can autonomously decompose tasks, by leveraging association rule mining, which discovers hidden relationship among entities in data mining. We introduce a novel method called ARM-HSTRL (Association Rule Mining to extract Hierarchical Structure of Tasks in Reinforcement Learning). It extracts temporal and structural relationships of sub-goals in RL, and multi-task RL. In particular,it finds sub-goals and relationship among them. It is shown the significant efficiency and performance of the proposed method in two main topics of RL.

==> document.tex <==
\section{Experimental Results}

\noindent In this section, three experimental results are presented on two testbeds, Figures \ref{testbed1} and \ref{testbedthreeima}, for ARM-HSTRL. The agent has 5 actions, $press-key$ and 4 movement primitive actions. The $press-key$ does not change the place of the agent. The agent can move with its primitive actions in four directions: $up$, $right$, $down$, $left$. If there is a wall in the way, the agent stays in its current state. In all of the experiments, if the agent does the $press-key$ in a wrong place, it receives the reward of $0$ in the sub-goal places and the reward of $-10$ in other states. The reward for other actions is $-1$. The agent movement with probability $0.8$ is according to intended action and is randomly in one of the directions with probability $0.2$. The discount factor was set to $\gamma$= $0.9$. 




\begin{figure}
	%\centering     %%% not \center
	
	\subfigure[]{\label{testbed1}\includegraphics[width=80mm, height=1.4in]{mazenew.PDF}}
	\subfigure[]{\label{testbedthreeima}\includegraphics[width=80mm, height=1.8in]{threetasks.PDF}}
	%	\subfigure[]{\label{Taxi}\includegraphics[width=40mm, height=1.4in]{Taxi.pdf}}	
	
	\caption{(a) The first testbed: the size of the maze is $22\times22$ and it has 7 sub-goals. Subgoals are colored with yellow. (b) The second testbed: the size of the maze is $26\times26$. Each task has 5 sub-goals and is shown with a different color.}
\end{figure}

